What we see and What we don't see: Imputing Occluded Crowd Structures from Robot Sensing

We consider the navigation of mobile robots in crowded environments, for which onboard sensing of the crowd is typically limited by occlusions. We address the problem of inferring the human occupancy in the space around the robot, in blind spots, beyond the range of its sensing capabilities. This problem is rather unexplored in spite of the important impact it has on the robot crowd navigation efficiency and safety, which requires the estimation and the prediction of the crowd state around it. In this work, we propose the first solution to sample predictions of possible human presence based on the state of a fewer set of sensed people around the robot as well as previous observations of the crowd activity.

==> followbot.tex <==
% !TeX root=main.tex

\section{Follow Bot}
The purpose of the Followbot project is to build a robotic framework including perception, prediction and navigation blocks in order to develop and evaluate the crowd prediction capabilities from the robot perspective.

As you see in Fig \ref{fig:followbot_pipeline} in this system we consider the input signals to come from a 2D LiDAR sensor. The range data are processed by a deep person detection module (DROW) and then a tracking module that filters the detections.

The tracks are fed into the crowd prediction module and the output is a Temporal Expected Occupancy Map (TEOM). This data is then used in navigation module.

\begin{figure*}
	\centering
	\includegraphics[trim={0 0 0 0},clip, width=0.9\textwidth]{../figs/followbot-pipeline.png}
	\caption{FollowBot pipeline}
	\label{fig:followbot_pipeline}
\end{figure*}


==> pcf_gp.tex <==
% !TeX root=main.tex

\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\mvec}[1]{\mathbf{#1}}

\def\delequal{\mathrel{\ensurestackMath{\stackon[2pt]{=}{\scriptstyle\Delta}}}}
\def\BibTeX{{\rm B\kern-.05em{\sc i\kern-.025em b}\kern-.08em
		T\kern-.1667em\lower.7ex\hbox{E}\kern-.125emX}}

\section{Using Gaussian Processes}

Let us assume that we have been able to learn, from a training stage and the observation of multiple example trajectories, a prior PCF, namely a function $\pi_0(r)$ of the radius.

We will attach to this function a Gaussian Process, defined by its mean function $m(r)$ and its covariance function $k(r,r')$
\[
\begin{array}{rcl}
    m({r}) & \delequal & E[\pi({r})]\\
    k({r},{r}') & \delequal & E[ ( \pi({r})-m({r}) )( \pi({r}')-m({r}') ) ].
\end{array}
\]
Then, we choose $m(r)=\pi_0(r)$ and write that our unknown PCF follows the Gaussian process 
\[
\pi(r) \sim GP(m(r),k(r,r')) .
\]

The function $k$ (\textit{kernel})  measures the similarity to other observations of the output of the function $\pi$ at a point $r'$, with respect of the closeness of $r'$ with the rest of the $r$ that have generated those observations. A commonly used covariance function is the \textbf{squared exponential} 
$$ 
k(r,r') = \sigma^2 \exp ( \frac{-(r-r')^2}{2l^2} )
$$
where $\sigma^2$ is a covariance and level $l$ is a length parameter. 


Now, at a given frame, we can observe a set of $n$ noisy values $\mvec{p}=\{({r}_i,p_i)\}_{i=1}^{n}$, where $p_i$ is the corresponding scalar target value to $r_i$. We assume that each $p$ is a noisy observation of the value of some true (but unknown) function $\pi({r})$ 
\[    p = \pi({r}) + \epsilon,   \]
where $\epsilon$ is Gaussian noise
\[   \epsilon \sim \mathcal{N}(0,\sigma^2).   \]

Hence for each $i=1,\hdots,n$ we have that
\[ p(p_i|r_i) = \mathcal{N}(p_i|r_i, \sigma^2). \]
As each observation is independent from the others, the joint distribution of $\mvec{p}$ will be
\[p(\mvec{p}|\mvec{r}) = \mathcal{N}(\mvec{p}|\mvec{r}, \sigma^2\mvec{I}). \]
And, as we saw before, the marginal distribution of $\mvec{p}$ will have zero mean and covariance $\mvec{K}'$
\[ p(\mvec{p}) = \mathcal{N}(\mvec{p}|k_0(\mvec{r}), \mvec{K}'), \]
where
\[ \mvec{K}' = 
\begin{bmatrix}
    k(r_1,r_1) &  k(r_1,r_2) & \hdots & k(r_1,r_n) \\
    \vdots & \vdots & \ddots & \vdots \\
    k(r_n,r_1) & k(r_n,r_2) & \hdots & k(r_n,r_n) 
\end{bmatrix}.
\]
Adding noise let $\mvec{K} = \mvec{K}' + \sigma^2 \mvec{I}$. And n
\[ \mvec{K}' = 
\begin{bmatrix}
    k(r_1,r_1)+\sigma^2 &  k(r_1,r_2) & \hdots & k(r_1,r_n) \\
    \vdots & \vdots & \ddots & \vdots \\
    k(r_n,r_1) & k(r_n,r_2) & \hdots & k(r_n,r_n)+\sigma^2 
\end{bmatrix}.
\]
Then the marginal distribution of $\mvec{y}$ is given by
\[ p(\mvec{p}) = \mathcal{N}(\mvec{y}|k_0(\mvec{r}),\mvec{K}'). \]
Now, given a new set of values ${r}_*$, we want to find the predictive distribution of the noiseless target value $p_*$, $ p(p_*|\mvec{p})$.  Let $\mvec{r}_* = [r_1,r_2,\hdots,r_n, r_*]$ and $\mvec{p}_* = [p_1,p_2,\hdots,p_n, p_*]$ then the joint distribution over $p_1,p_2,\hdots,p_n, p_*$ will be
\[ p(\mvec{p}_*) = \mathcal{N}(\mvec{p}_*|k_0(\mvec{r}_*), \mvec{K}_*) \]
where
\begin{equation}
    \mvec{K}_* = 
\begin{bmatrix}
    k(r_1,r_1)+\sigma^2& \hdots & k(r_1,r_n) & k(r_*,r_1)\\
    \vdots & \ddots & \vdots & \vdots \\
    k(r_n,r_1) & \hdots & k(r_n,r_n)+\sigma^2 & k(r_*,r_n)  \\
    k(r_*,r_1) & \hdots & k(r_*,r_n) & k(r_*,r_*) 
\end{bmatrix} = 
\begin{bmatrix}
    \mvec{K} & \mvec{k}\\
    \mvec{k}^T & c
\end{bmatrix}
\end{equation}
and
\[
\begin{array}{lr}
    
\mvec{k} =
\begin{bmatrix}
    k(r_*,r_1)\\
    \vdots \\
    k(r_*,r_n)
\end{bmatrix} 
&  c = k(r_*, r_*).\\
\end{array}
\]
Thus we get the conditional distribution as
\[ p(p_*|\mvec{p}) = \mathcal{N}(p_*|\mu_*, \sigma_*^2) \]
with mean and covariance
\begin{equation}
 \mu_* = \pi_0(r_*)+\mvec{k}^T \mvec{K}^{-1}(\mvec{p}-\pi_0(\mvec{r}))
\label{mean}
\end{equation} 
\begin{equation}
 \sigma_*^2 = c - \mvec{k}^T \mvec{K}^{-1}\mvec{k}.
\end{equation} 
The estimate for the value of the CFP at $r_*$ will be the mean $\mu_*$ and the uncertainty of this prediction will be $\sigma_*^2$. \\ `


==> proposed_old.tex <==
% !TeX root=main.tex

\section{Proposed Method}
\label{sec:proposed}

Suppose that a robot navigates in an environment shared by $n$ pedestrians, each of which being represented by its position $\mathbf{x}_i\in \mathbb{R}^2$ and its instantaneous velocity $\mathbf{v}_i\in \mathbb{R}^2$. The robot uses its sensors to get raw measurements and passes them to a human detection unit that returns a set of $m$ detections as ${\mathbf Z} = \{\mathbf z_1, ..., \mathbf z_{m} \}$ (see Fig. \ref{fig:multi-social-object-tracking}), which are noisy observations of the positions $\mathbf{x}_i$. 

We assume there are $u=n-m$ unobserved pedestrians, either due to errors by the detector or because the pedestrians are not visible by the sensors, e.g. because of an occlusion or because they are out of the robot field of view.

To impute the position of unobserved pedestrians, our algorithm leverages the information about geometric relations between the people in the surrounding crowd, so that we can improve the robot's knowledge about the environment and build more reliable motion plans estimate and plan beyond what it can see. Before detailing our imputation algorithm, we first introduce the concept of Social Tie.

\begin{figure}
	\centering
	\includegraphics[width=0.95\linewidth]{"../figs/multi social object tracking"}
	\caption{The graphical representation for Occlusion- and Socially-aware Object Tracking. The yellow circles show the state of each agent at two consequent time instants $t-1$ and $t$. The blue circles are the observations at current time instant $t$. The dashed green arrows represent the social interaction between the agents and the blue arrows represent the observation model.}
%	\CommentJB{Switch from k to t?}
%	\CommentJvd{I'll fix it}
	\label{fig:multi-social-object-tracking}
\end{figure}


\subsection{Social Ties}
\label{subsec:ST}

The idea of extracting patterns from collective behaviors has a long history. For example, Moussaid et. al~\cite{moussaid2010walking} have studied the grouping behavior on crowd videos recorded in public places and have reported the patterns such as group sizes and the distance and angle between the group members. Alahi et. al \cite{alahi2014SAM} have later created a huge dataset of human trajectories, recorded in a train station, and have proposed \textit{Social Affinity Maps (SAM)} to capture the spatial position of an agent’s neighbors by radially binning the positions of his neighboring agents. In fact, they end up with a 10-bit binary radial histogram which is suggested to be a robust feature, not changing frequently and significantly over time. This feature improves the re-identification of groups in consequent \textit{tracklet}s extracted from different cameras in the train station.

Inspired by these works, we propose a basic definition of a Social Tie, as a displacement vector between a pair of agents $i$ and $j$, expressed in the local frame of the first one: 

\begin{equation}
	\delta({\textbf{x}}_i, {\textbf{x}}_j) = (\textbf{R}_{i})^\top ({\textbf{x}}_j - {\textbf{x}}_i),
	\label{eq:social-tie}
\end{equation}

\noindent
where $\textbf{R}_{i}$ is the rotation matrix giving the global orientation angle of agent $i$ in the current timestep.

We further classify the social ties as \emph{strong ties} and \emph{absent ties}. The terms are borrowed from social networks literature~\cite{granovetter1973ties} to represent, respectively, long-term interactions (e.g. grouping or leader-follower behaviors) versus instant interactions (e.g. collision avoidance overtaking) between pair of agents.
%
The motivation behind this modeling choice is that these two categories (strong/absent) define different distributions of displacements $\delta$, which we refer to as $\delta^S$ and $\delta^A$, respectively, that are better to be treated dissimilarly. 

The classification between the two tie types is based on the history of the distance between two agents. We keep the history of the distance vector between all pairs of detected agents. 
%
A tie is labeled as \emph{strong}, if 1) during the last $t_{c}$ time-steps, the two agents are closer than a threshold distance $r_{max}$, 2) in the same time interval, the Euclidean distance between the agents remains fixed (up to a \hl{tolerance threshold $\epsilon_l$} [JBH: tolerance on what?]) over the last second, and 3) the agents have similar orientations (within another threshold $\epsilon_{\theta}$). If 1) holds but either 2) or 3) does not, then the link is categorized as absent.
While we found these simple rules to be enough in our setup, more advanced classification rules can also be used. An example is depicted in Fig.~\ref{fig:ties_classification_rule} to illustrate the classification process.

The above definition implies that a tie (strong or absent) is assigned to any pair of agents that have a distance lower than $r_{max}$ during the last $t_{c}$ time-steps.
%
It is worth observing that the tie definition is symmetric: a strong (absent) tie from $\textbf{x}_i$ to $\textbf{x}_j$ implies a strong (absent) tie from $\textbf{x}_j$ to $\textbf{x}_i$. However this symmetry property is not directly implied by the definition of social tie, but by the classification rule, which means with a new classification method, one-way ties may exist. 


%\CommentJvd{In the last 1.0 sec, no change in distance more than 0.5 meter, and with difference between orientations not more than 45 degree}

\begin{figure}[!htb]
	\centering
	\includegraphics[trim= 6 25 6 25, clip, width=0.9\columnwidth]{"../figs/Social Ties"}
	\caption{
		Social Ties. The tie between $\mathbf{x}_1$ and $\mathbf{x}_2$ is classified as a \textit{strong} tie at time $t$, (shown in green). On the other hand, the link between $\mathbf{x}_2$ and $\mathbf{x}_3$ is \textit{absent} (red dashed line)
%		 due to significant change from $t-1$ to $t$
		.
	}
	\label{fig:ties_classification_rule}
\end{figure}

The next step is to compute the distribution of the social ties. This is done by classifying and accumulating the observed ties and then taking the polar histogram of each one. The two histograms represent the empirical distribution of the strong and absent ties. They are denoted by $p(\delta^S|\mathcal{H})$ and $p(\delta^A|\mathcal{H})$, respectively, where $\mathcal{H}$ denotes the historical observations used for training.
%
Observe that these distributions on displacements give us access to the conditional distribution of the absolute location of a queried pedestrian $\textbf{x}_q$, conditioned on seeing a first pedestrian $\textbf{x}_i$, and on the type of social tie $\delta$, i.e., $p(\textbf{x}_q|\textbf{x}_i, \delta, \mathcal{H})$.

Some examples are shown in Fig.~\ref{fig:p-ties}, where one can observe that the different collective patterns of pedestrians have led to significantly different social tie patterns in the Bottleneck and ETH (Zara) Datasets. These distributions can help us in estimating the location of people in unseen (occluded) areas. We will discuss this in the following.

% The assumption is that a untracked agent holds ties with other pedestrians that follow the obtained distribution.

%\hl{Intuitively, grouping and following behavior patterns will be captured in strong ties, and other transient interactions such as passing, crossing or overtaking will appear in the absent ties} 

%\textit{Implementation tips:}
%The distributions are calculated using polar histograms over the observed ties. We only keep the ties at a distance shorter than a radius $R_{max}$. An example distribution is shown in Figure \ref{fig:p_link} for a simulated crowd that is composed of bi-directional flow of agents, moving in groups of size 2.

%\begin{figure}[tb]
%\centering
%\includegraphics[width=0.9\linewidth]{../figs/p_link}
%\caption{Distribution of Pairwise links for a Bidirectional simulated crowd 
%\CommentJB{Is it for strong ties? or for absent ties?}}
%\CommentJvd{arg1}
%\label{fig:p_link}
%\end{figure}


%\subsubsection{Filtering irrelevant values}

%During a crowd activity scenario, the configuration of the agents usually change at every frame. Parts of the data calculated from these configurations may be misleading. For example, the trajectories of 2 persons moving in opposite directions will generate in Eq.~\ref{eq:tpcf} a sequence of distances, which starts with a higher distance, then decreases down to a minimum distance $\min_t(d_{i, j})$ and then increases again. From only this single sequence, we would end up with a uniform distribution of distances.
%
%We modified the temporal pair correlation function defined above to use the minimum observed distance between each pair of pedestrians, instead of the average value.
%
%* [\hl{Formal definition}]
%
%We will finally compute a discretized PCF, such that the functions are evaluated at $r_1, ..., r_k$. This gives a vector of real-valued numbers:
%$\phi = [TPCF(r_1) ... TPCF(r_1)]^T$

%\CommentJB{To discuss, I feel this lead to a very pessimistic estimation of the state of the crowd?}


%\hl{todo:}
%
%\begin{itemize}
%	\item[\checkmark] classify detected motions into F flows
%	\item[\checkmark] extrapolate the flows to blind spots
%	\item[\checkmark] compute distribution of distances for each flow (analysis)
%	\item[4.] create $H$ hypothesis in blind spots, by adding synthetic agents
%	\item[5.] use predict/update scheme in Kalman Filter to update the state of system
%\end{itemize}

%\subsection{Velocity Distribution}
%For capturing the velocity distribution, we fit a GMM (Gaussian Mixture Model) at any point $\textbf{x}$ of the the environment:
%
%\begin{equation}
%\textbf{v}(\textbf{x}) \sim \sum_{i}^{N} \textbf{w}_i \mathcal{N}(\mu_i, \Sigma_i).
%\end{equation}
%
%\CommentJB{Give details; N is fixed? Depends on x?}

\subsection{Communities (clusters)}
\label{subsec:Flows}
%By imagining an untracked agent at an invisible location $\textbf{x}_i$, we have assumed this pedestrian holds tie to every other person in the environment, either strong or absent. This implies that this set of $N$ ties can have $2^N$ different configuration. The concept of communities is presented to make this problem simpler.

We define \textit{communities} as subsets of pedestrians that are connected (directly or indirectly) by strong ties, i.e., that can be seen as clusters of people moving together as a group, or a continuous flow of people moving in one direction (see examples in Fig.~\ref{fig:communities}).
The $m$ observed agents will be partitioned into $K$ communities: $\textbf{C} = \{\textbf{c}_1, ..., \textbf{c}_K\}$. A community can be as small as containing only one person.
The velocity of community $\textbf{c}_k$ is defined as the average velocity of its members:
\begin{equation}
	\textbf{v}_k = \frac{1}{|\mathbf c_k|} \sum_{i \in \mathbf c_k}{\textbf{v}_i}
\end{equation}

We also define a territory area for each community, by running a k-nearest neighbor classifier that assigns to every location a label that represents the nearest community. The probability of being, at a location $\mathbf x$, in the territory of $c_k$ is denoted by $\phi^{c_k}(\mathbf x)$.

%Then an untracked agent will be member of one of these communities or is from an untracked community. Then the number of configurations will drop to $K+1$ (the agent will have strong ties to members of a community, and hold absent ties to persons from other communities).


\begin{figure*}
	\begin{center}
		\begin{tabular}{cc}
%			\includegraphics[trim= 60 60 55 35, clip, width=0.3\linewidth]{../exp/links/HERMES-bo-360-075-075-0155}& 
			\includegraphics[trim= 121 0 90 50, clip, width=0.56\linewidth]{../figs/territories-Hermes}

%			\includegraphics[trim= 60 40 30 35, clip,width=0.35\linewidth]{../exp/links/ETH-Hotel-0181}
			\includegraphics[trim= 60 0 60 50, clip,  width=0.4\linewidth]{../figs/territories-zara}

		\end{tabular}
	\end{center}
	\caption{Communities. Green lines: strong ties, red lines: absent ties, and blue lines: velocity vector of the agents. Left: Bottleneck dataset, a bi-directional flow of pedestrians that form two communities, Right: Hotel dataset with 3 communities moving in different directions}
	\label{fig:communities}
\end{figure*}

%By classifying social ties between agents as we have shown above, we construct multiple connected components that move in a \textit{crowd flow}. 
%\CommentJB{Only strong ties?}.
%\CommentJvd{Yes. A set of agents that are connected with strong ties (Fig. \ref{fig:classify-ties})}
%The set of connected agents, assigned to $\Phi_i$ 
%\CommentJB{What is phii? }is shown by $\{X^{\Phi_i}\}$ \CommentJB{I dont understand the notation}. We then use a nearest-neighbor classifier to assign the flow class of the nearest agent to a given location $\textbf{x}$. This categorical variable which is shown by $\Phi(\textbf{x})$ will help us to predict and generate virtual agents, explained the next section.
%
%\CommentJB{Some confusion about the notion of classification: Above you described a classification into strong/absent. Is it the same you are talking about here?}

%\begin{figure}
%\centering
%\includegraphics[width=0.9\linewidth]{../exp/flow/crowd_flow_map}
%\caption{Above: ground truth agents from Bottleneck Dataset. Bottom: detected and tracked agents by the robot (black circle) and two classes of flows shown by red and blue.}
%\label{fig:crowd_flows}
%\end{figure}


\subsection{Projecting New Pedestrians}
\label{subsec:Virtual}

We explained in~\ref{subsec:ST} that the social ties are extracted from crowd activity observations. Here we leverage this data to predict plausible positions for the unobserved agents that might exist in the blind spot areas and beyond the field of view of the sensor. This idea is inspired by \textit{Inpainting} technique in Computer Graphics, where Pair Correlation Functions (PCF)~\cite{nicolet2020pcf} are used to detect textures from an image and propagate them to other areas.
%The PCF of a set of 2D points is computed as follows:
%\begin{equation}
%\mathbf{PCF}: \phi(r) = \frac{\rho_r}{N-1} \sum_{i \neq j}^{N} k_{\sigma} (r- \lVert \mathbf{x}_i - \mathbf{x}_j \rVert)
%\label{eq:pcf}
%\end{equation}
%\noindent where $N$ is the number of particles/agents, $k_{\sigma}(x)=\frac{1}{\sigma \sqrt{2\pi}} e^{-x^2 / 2\sigma^2}$ is a Gaussian kernel, and $\rho_r$ is a normalization factor equal to 1 over the area of a ring with inner radius $r - 0.5$ and outer radius $r + 0.5$. \CommentJB{So the normalization factor cannot be defined for values inferior to 0.5?}
A PCF measures the probability density of the distance between pairs of particles. However, in our context, considering only the distance between agents is difficult, since the orientation of the agents is critical in modeling human collective activities~\cite{moussaid2010walking}. Hence, we propose an extension of the concept of PCF with the distribution of social ties.

%\CommentJvd{A new story:}\\
Suppose $\textbf{X}$ to be the current state of the crowd i.e., the set of locations of the tracked agents. 
We are interested in finding 
$p(o(\mathbf{x}_q)|\mathbf{X}^d)$
which represents the probability of the presence of another, unobserved agent 
at query point $\textbf{x}_{q}\in \mathbb{R}^2$, given the positions of the robot and the other/\hl{detected} agents $\mathbf{X}^d$.
%
This distribution is a sum of \hl{Dirac} functions at the location of agent in $\textbf{X}$.
%
By \hl{marginalizing} this distribution on two latent variables $v$ and $\mathbf c$ for, respectively, the visibility from the robot at position $\mathbf x_q$ and the class indicating the community at that position, we can write this as (we dropped the $\textbf{x}_{q}$ for keeping it short):

{\small
\begin{align}
	 p(o|\mathbf X^d)&=& \sum_{w\in \{0,1\}} \sum_k  p(o , \mathbf  c=\mathbf c_k, v=w |\mathbf{X}^d)&\\
% 	&=& \sum_k  p(o, \mathbf  c=\mathbf c_k, v=0 |\mathbf{X}),&\\
% 	&=& \sum_k  p(v=0|\mathbf r) p(o, \mathbf  c=\mathbf c_k|\mathbf{X}), &\\
	 &=& p(v=0) \sum_k  p(\mathbf  c=\mathbf c_k) p(o| \mathbf  c=\mathbf c_k,\mathbf{X}^d).
	 \label{eq:marginalized-2}
\end{align}
}

Using the community-dependent ties distributions, we  estimate $p(o| \mathbf  c=\mathbf c_k,\mathbf{X}^d)$ as follows:

\begin{align}
\begin{split}
	\hat p(o| \mathbf c_k,\mathbf{X}) =
	\prod_
	%	{\textbf{x}_i \in \{X^{\Phi(\textbf{x}_q)}\}}
	{i \in \mathbf X \cap \textbf{c}^k}
	p(\delta^S(\textbf{x}_i^t, \textbf{x}_{q}) |\mathcal{H}) \\
	\times
	\prod_
	%	{\textbf{x}_j \notin \{X^{\Phi(\textbf{x}_q)}\}}
	{j \in \mathbf X \backslash \textbf{c}^k}
	p(\delta^A(\textbf{x}_j^t, \textbf{x}_{q}) |\mathcal{H})
\end{split}	
\end{align}

where 
$p(\delta(\textbf{x}_i^t, \textbf{x}_q)|\mathcal{H})$ denotes the likelihood of a social tie between $\textbf{x}_i$ and a person at position $\textbf{x}_q$ and time $t$, which has been constructed with historical data $\mathcal{H}$.
%
\hl{The estimation is based on considering only joint distribution of two agents.}
%
In practice, we only consider the agents in $\textbf{X}$ in radius $r_{max}$ from $\textbf{x}_q$.
%
Finally we can rewrite Eq. \eqref{eq:marginalized-2}, using the notation introduced above $\phi^{c_k}=p(\mathbf  c=\mathbf c_k)$:

\begin{equation}
	\hat p(o|\mathbf X^d) =
	p(v=0)
	\sum_{k}
	\phi^{c_k} 
	\hat p(o| \mathbf  c=\mathbf c_k,\mathbf{X}^d)
\label{eq:product_p(ties)} 	
\end{equation}


%The product in the equation above is performed after rotating the polar histogram $p(\delta)$ toward direction of each agent and then converted to Cartesian form. In the areas out of histogram bound, we pad the probability with $\bar p = mean(p(\delta))$. \CommentJB{Not very clear.}
%In Alg.~\ref{alg:crowd-pred-init}, we describe the overall process of crowd synthesis and prediction for the robot. 
%The inputs of this process are two Probabilistic Occupancy Maps (POM) $\pi_0$ (from the data) and $\pi^t_{r}$ (from the robot's Lidar at time $t$).
%
%At initialization, we update $\pi_0$ with the first perception $\pi_r^0$ to get the posterior POM $\pi_f^0$. \CommentJB{I guess that the perception process is able to segment the LIDAR scan into $\pi_r^0$ (static map) and $\textbf{x}_{d}^0$ (mobile agents), right?} Having detected the mobile agents around robot, $\textbf{x}_{d}^0$, we apply the \emph{DartThrowing} algorithm in Alg.~\ref{alg:dart-throwing} for $K$ times to get $K$ different sample sets of synthesized agents $\textbf{s}^{0}_{k}$ for $1 \leq k \leq K$.
%
%Then, at each time-step of the navigation loop of the robot, we update all synthetic and detected agents, using multi-modal prediction function \emph{Pred}. This function (as a generative model) takes a random input $\textbf{z}_j$ and gives a prediction output; repeated $N_{pred}$ times, this gives us $N_{pred}$ different prediction outputs: $\textbf{\^s}_{k, j}^{t:t+T_{p}}, \textbf{\^x}_j^{t:t+T_{p}}$ for, respectively, the simulated agents and the tracked agents. These $N_{pred} \times K$ synthetic agents are ranked and sorted to select the top $K$ items for next iteration \CommentJB{A bit vague. I assume that in some way you need to explore the $K^{N_pred}$ joint trajectories?}. By calculating a POM for all $K$ synthetic samples and detected agents, we achieve an Temporal POM estimation for next $T_p$ time window. \CommentJB{Could see to keep several POMs?}
%


%\subsection{Reconstruction Algorithm} 
%
%The purpose of the reconstruction algorithm is to make multiple guesses (samples) about blind spots of the crowd, using the already extracted pattern (PCF).
%
%
%
%%\noindent
%\textbf{\textit{Original Dart throwing}}:
%
%In this algorithm, at each time-step, a random point is generated. If the distance of this point to the closest point in the set of already accepted points is smaller than desired \CommentJB{Explain what 'desired' mean}, it is rejected and otherwise it is accepted.
%
%\textbf{\textit{C. Generalized Dart throwing}}:
%The algorithm is an extension of original dart throwing algorithm, by using pair correlation functions~\cite{oztireli2012gendartthrowing} instead of fixed desired radius values. For a given target PCF $\phi_0$, one can simply impose the condition that at any given iteration: $TPCF(r_k) \leq \phi_0(r_k) ~ \forall r_k$. 
%Given the explanation about not normalizing the TPCF in Eq. \ref{eq:tpcf}, we propose Algorithm~\ref{alg:dart-throwing}.
%
%
%\begin{algorithm}
%	
%	\caption{Customized Dart Throwing\label{alg:c-dart-throwing}}
%	
%	\hspace*{\algorithmicindent} \textbf{Input}: $\phi_0$ (target TPCF), $X_0$ (Observed Points), K (limit of samples)
%	
%	\hspace*{\algorithmicindent} \textbf{Output}: $X_{out}$ 
%	
%	
%	\begin{algorithmic}[1]
%		\State $X_{out} \leftarrow X_{0}$ \Comment{Initialize}
%		\State $Z = X_{out}$ \Comment{Active List}
%		
%		\While{$Z \neq \emptyset$}
%		\State{$ x_{parent} \leftarrow \mathrm{DrawFromActiveList}()$}
%		\State{$r_c \leftarrow \mathrm{ChooseMinDist(\phi_0)}$}
%
%		\For{k in 1..K}
%		\State{$x_{new} \leftarrow \mathrm{UniformRandom(Disk(r_c, 2 r_c))}$}
%		\If{$ \min_i ||x_{new} - X_{out}^i|| > r_c$}
%		\State $X_{out} \leftarrow X_{out} \cup x_{new}$
%		\Comment{Accept}
%		\State $Z \leftarrow Z \cup x_{new}$
%		\EndIf
%		\EndFor
%		
%		\If{$\mathrm{FailedToAdd}$}
%		\State{$Z \leftarrow Z \char`\\ x_{parent}$}		
%		\EndIf
%			
%		\EndWhile
%	\end{algorithmic}
%\end{algorithm}
%
%\begin{algorithm}
%	
%	\caption{Generalized Dart Throwing\label{alg:dart-throwing}}
%
%	\hspace*{\algorithmicindent} \textbf{Input}: $\phi_0$ (target TPCF), $\pi_0$ :POM, $N_{try}: int, X_{0}$: (Observed Points) 
%		
%	\hspace*{\algorithmicindent} \textbf{Output}: $X_{out}$ 
%	
%	\begin{algorithmic}[1]
%		\State $i \leftarrow 0$ \Comment{iterator}
%		\State $X_{out} \leftarrow X_{0}$
%		
%		\While{$i < N_{try}$}
%		\State $i \leftarrow i+1$
%		\State{$ x_{new} \leftarrow \mathrm{DrawRandomPoint}(\pi_0)$}
%		\State{$ \phi_{new} \leftarrow \mathrm{CalcPCF}(X_{out} \cup x_{new})$}
%		
%		\If{$ \min_r(\phi_{0}(r)-\phi_{new}(r))>0$}
%		\State $X_{out} \leftarrow X_{out} \cup x_{new}$
%		\Comment{Accept}
%		
%		\Else
%		\State{$g_{new} \leftarrow \sum_{r ~st~ \phi_{new}^r > \phi_0^r} (\frac{\partial \phi_{new}^r}{\partial x_{new}})$}
%
%		\State{$ x_{new} \leftarrow x_{new} -\alpha g_{new} $}
%		\Comment{Gradient Descent}
%		\State {Repeat Lines~6:8}
%		\EndIf
%		\EndWhile
%	\end{algorithmic}
%\end{algorithm}
%
%
%An example of reconstruction by Dart throwing in Fig. \ref{fig:pcf-GC-2066} 
%
%
%\begin{figure*}
%	\centering
%	\includegraphics[width=0.99\linewidth]{../plots/pcf-example-GC-2066}
%	\caption{}
%	\label{fig:pcf-GC-2066}
%\end{figure*}

%\subsubsection{Sampling by Poisson Distribution!!!}


%\hl{todo: Isn't it enough to have strong ties to only q closest people of the community $N_{C^k}$}



%\subsection{Iterative Sampling 
%	+ Refining
%% the projections from past predictions
%	}

By sampling from this distribution we can project/\hl{impute} a new agent at location $\mathbf{\hat x}_v$, which should ideally be equal to the location of one of the undetected agents.
%
We tested different \hl{sampling strategies}, and found out the following sampling to be more effective: we draw a sample from $\hat p$ and then we search within a small circle $r_s$ for the highest probability value, i.e. the local maximum of $\hat p$ in this region.
%
After this, a \textit{\hl{virtual}} agent will be created at this location, and assigned to community $\argmax_{\textbf{c}_k} p(\textbf{c}=\textbf{c}_k)$, with velocity $\textbf{v}_k$.
%
By iterating the sampling, we will create more agents in the occluded area. After sampling iteration $\#i$, we add $\mathbf{\hat x}^{(i)}_v$ to $\mathbf{\hat X}^{(i-1)}$ (having $\mathbf{\hat X}^{(0)}\equiv\mathbf{X}^{d}$) and update $\hat p^{(i)}$ using Eq. \eqref{eq:product_p(ties)}.
%
%\hl{How many times we do this process?}
We repeat the process until $\max_{\textbf{x}_q} \hat p < \epsilon_s$ in a $r_{nav}$ neighborhood around the robot.


\subsection{Multiple-Hypothesis Prediction}
By repeating the sampling process, explained in the previous section, for $w$ times, we will achieve $\mathbf{\hat X}^{(w)}$ as the set of all detected and projected agents. We repeat this entire process, for $H$ times to get multiple set of hypotheses $\mathbf{\hat X}^{(w, h)}$. These hypotheses ...

The complete prediction algorithm can be found in Algo.\ref{alg:overall}.
%\CommentJvd{Change Synthetic $\rightarrow$ Projected}
%As we saw above, the most straightforward interaction between crowd synthesis and pedestrian prediction is by feeding the prediction algorithm with synthetic data such that the future motion is determined by taking into account potential unseen obstacles in front of an agent. The interaction can also work the other way round: As the prediction depends on the synthesis, we can use discrepancies between the observed trajectories by an agent and the predicted one (a few frames before) to adapt/refine the position of the synthetic agent\dfrac{num}{den}s. More formally, let us consider one agent $i$. Its observed trajectory up to $t$ is:
%
%$$
%\mathbf x_i^{1:t}
%$$
%
%\noindent and the predictor will use the positions of the other observed agents $j$ at $t$, $\bar{\mathbf x}_{j}^t$ and the positions of the synthetic agents, that we will denote as $\tilde{\mathbf x}_{l}^t$ to perform the prediction about $\mathbf x^{t+1:t'}_i$ as
%
%$$
%\hat{\mathbf x}^{t+1:t'}_i = \pi(\mathbf x_i^{1:t},\{\bar{\mathbf x}_{j}^t\}_{j},\{\tilde{\mathbf x}_{l}^t\}_l).
%$$
%
%Then, once new observations come about $i$, we will be able to compare these observations to the predictions that were made, and evaluate
%
%$$
%\|\hat{\mathbf x}^{t+1:t'}_i-{\mathbf x}^{t+1:t'}_i\|^2 = \|\pi(\mathbf x_i^{1:t},\{\bar{\mathbf x}_{j}^t\}_{j},\{\tilde{\mathbf x}_{l}^t\}_l)-\mathbf x^{t+1:t'}_i\|^2
%$$
%
%\noindent and minimize this quantity seen as a function of the $\{\tilde{\mathbf x}_{l}^t\}_l$ i.e. by gradient descent (using numerical derivatives).
%
%
%%keeps two types of tracks or agents:
%
%\begin{itemize}
%	\item[\textit{A}.] Normal tracks $\bar{\textbf{x}}^t$: those are tracks about the state of agents that have been previously associated to at least one detection,
%	\item[\textit{B}.] \textit{Virtual} agents $\tilde{\textbf{x}}^t$: those are tracks about agents that have never been detected but are instead inferred/projected by the robot as predictions in blind spot areas. We will describe these in more detail in the following.
%\end{itemize}
%




%\subsection{Interaction-Aware Trajectory Prediction}
%The state of each agent $i$ at time $t$, either normal or virtual, is denoted by not-accented $\textbf{x}^t_i$ letter. We suppose that this state evolves following a \textit{social} motion model $f$:


%\begin{equation}
%\textbf{\^x}^{t}_i = 
%f(\textbf{x}^{t-1}_i, \bigcup_{j\neq i}{\textbf{x}}^{t-1}_j) 
%+ v_i
%\end{equation}

%\noindent where $v$ is a process noise, assumed to be white, zero-mean, Gaussian, with a covariance matrix $Q$. The motion model $f$ is dependent on the state of other agents because of the social interactions between the agents (avoidance, grouping, pursuit\dots). This dependency is depicted through the dashed-green arrows in Fig.~\ref{fig:multi-social-object-tracking}

%At each timestep, the assignment of detections $\mathbf z$ to the closest agents $\mathbf x$ is done using Munkers algorithm \cite{munkres1957}, where we use the euclidean distance between detections and the agents as cost matrix.
%\CommentJB{Agents: You mean their predicted positions?}
%\CommentJvd{Exactly}
%The pseudo-code of the main algorithm is given as Algorithm~\ref{alg:overall}.

\begin{algorithm}
	\caption{Occlusion-Aware Crowd Tracking}
	\label{alg:crowd-pred-init}
	
	\hspace*{\algorithmicindent} 
	\textbf{Inputs}: $\mathbf Z^t$
	\Comment{detected persons at $t$} \\
	\hspace*{\algorithmicindent} \hspace*{31pt} $\textbf{\^X}^t$
	\Comment{predicted tracks from $t-1$} \\	
	\hspace*{\algorithmicindent} 
	%
	\textbf{Output}: ${\hat\pi}^{t}$ 
	\Comment{predicted POM at $t$}
	
	\begin{algorithmic}[1]
		\State Assign detections $\mathbf Z^t$ to tracks $\mathbf{X}^t$ using \textit{Munkres} algo.
		\State Initialize new tracks for unassigned detections
		\State \hl{Change} status of Virtual tracks to Normal if they got assigned
		\State %$\textbf{X}^t \leftarrow$ 
		Update tracks based on assigned detections 
%		\CommentJB{Dont understand the notation with the arrow}
%		\CommentJvd{Assignment :-)}
		
		\State Compute Social-Ties between detections $\delta^S, \delta^A$ (Strong/Absent) Eq. \ref{eq:social-tie}
%		\State Update $p(\delta^S|\textbf{Z}^{1:t})$ and $p(\delta^A|\textbf{Z}^{1:t})$ Eq. (Todo: explain prior distribution and update policy)
		
		\State Calculate Communities (Connected Components)
		
		\State Project new pedestrians by iterative sampling
		
		\State \hl{Refine} virtual agents $\{\textbf{x}_v\}$ using Eq. \ref{eq:product_p(ties)}
		
%		\State Predict jointly the state (trajectory) of all agents (real+virtual) for $t+1:t+T$ Eq. \ref{eq:social-predict}  for each hypothesis
		
		\State Compute Occupancy Map and return $\mathbf{\hat{\pi}}^{t}$
		
		%		\For {$t \in [1, \infty)$}	
		%		\EndFor
	\end{algorithmic}\label{alg:overall}
\end{algorithm}
%The rest of the tracking steps are similar to standard MOT trackers:
%\begin{itemize}
%	\item Update existing tracks based on assigned detections,
%	\item Initialize new tracks for unassigned detections,
%	\item Confirm tracks if they have appeared in $\Gamma\%$ of recent frames
%	\item Delete tracks if they have remained unassigned for too long, while being posed within FOV of the robot. \hl{Explain here more clearly}
%\end{itemize}

==> test.tex <==
\def \c {c}
\def \x {x}
\def \z {z}
\def \cprim {\c^{\prime}}


\begin{equation*}
\label{eq:eq4}
L_{adv} = \underset{G} {\min} \, \underset{D} {\max} \, [\log (D(\x))+ \log (1-D(G(\z)))]
\end{equation*}


\begin{equation*}
\label{eq:eq1}
\underset{G} {\min} \, \underset{D} {\max} \, L_I(D,G)=L_{adv}(D,G)-\lambda I(\c;G(\z,\c))
\end{equation*}



\begin{equation*}
\label{eq:eq22}
I(\c,\x) = H(\c) - H(\c|\x) = \mathbb{E}[-\log(P(\c))]-\mathbb{E}[-\log(P(\c|\x))]
\end{equation*}



\begin{eqnarray*}
\label{eq:eq3}
I(\c;\,G(\z,\c)) 
&=&
	H(\c) - H(\c|G(\z,\c))\\
&=&
	 \mathbb{E}_{\x\sim G(\z,\c)}
		 [\mathbb{E}_{\cprim\sim P(\c|\x)}[\log P(\cprim|\x)]] 
	 + H(\c)\\
&=&
	\mathbb{E}_{\x\sim G(\z,\c)}
		[\underbrace{D_{KL}(P(.|x) \,||\, Q(.|x))}_{\geq 0} 
		+ \mathbb{E}_{\cprim\sim P(\c|\x)}[\log Q(\cprim|\x)]]+H(\c) \\
&\geq&
\mathbb{E}_{\x\sim G(\z,\c)}
	 [\mathbb{E}_{\cprim\sim P(\c|\x)}[\log Q(\cprim|\x)]]+H(\c)
\end{eqnarray*}


\begin{equation}
\begin{split}
&EMD(\textbf{X}_r, \textbf{X}_g) = \min_{\mathbf w \in \mathbb{R}^{n \times m}}
\sum_{i=1}^{n} \sum_{j=1}^{m}
\mathbf w^{ij} d(\mathbf{x}^i_r, ~\mathbf{x}^j_g)		\\
\mbox{s.t. } & \forall i,j \; \mathbf w^{ij} \geq 0, \sum_{k=1}^m \mathbf w^{ik} = \frac{1}{n} \mbox{ , }\sum_{k=1}^n \mathbf w^{kj} = \frac{1}{m}.
\end{split}
\label{eq_EMD}
\end{equation}

\pagebreak

